Confidence-based Event-centric Online Video Question Answering on a Newly Constructed ATBS Dataset

Deep neural networks facilitate video question answering (VideoQA), but the real-world applications on video streams such as CCTV and live cast place higher demands on the solver. To address the challenges of VideoQA on long videos of unknown length, we define a new set of problems called Online Open-ended Video Question Answering (O^2VQA). It requires an online state-updating mechanism for the solver to decide if the collected information is sufficient to conclude an answer. We then propose a Confidence-based Event-centric Online Video Question Answering (CEO-VQA) model to solve this problem. Furthermore, a dataset called Answer Target in Background Stream (ATBS) is constructed to evaluate this newly developed online VideoQA application. Compared to the baseline VideoQA method that watches the whole video, the experimental results show that the proposed method achieves a significant performance gain.

==> sections/Experiments.tex <==
\section{Experiment}
%\textcolor{blue}{ATBS}
%\textcolor{green}{BridgeFormer}

In this section, the proposed method is compared with existing models for offline VideoQA
on our \textcolor{blue}{ATBS} dataset. The experimental settings are described. And how we adapt the offline methods to be compared is justified. The experimental results demonstrate that our method is able to localize the target information on online videos and achieve superior performance.

\subsection{Implementation Details}
As OVQA is a challenging and novel video question-answering task, there are no existing models as benchmarks. Thus, we adapt ALPRO \cite{li2022align_alpro}, the SOTA VideoQA model, to the OVQA task. Comparing our method of watching part of video, we conduct that ALPRO is allowed to encode the entire video. For being fairly comparable with our method, the same-sized frames are randomly sampled into the baseline model.  



\subsection{Experiment Settings}
The proposed method is compared with the baseline model in the offline setting 
to demonstrated superiority. 
The video-text retrieval model \textcolor{green}{BridgeFormer} \cite{ge2022bridging_video_text_retrieval} used in our method is initialized using official released weight and remained fixed.
\footnote{https://github.com/tencentarc/mcq}
For time saving, we firstly retrieval the dataset videos using our \textcolor{blue}{confidence-based target event localization} algorithm with 4 frame per seconds and record the founded target range. We set confidence threshold \textcolor{blue}{$\bm{c}_{max}$} to 0.4 and 
\textcolor{blue}{$\bm{c}_{min}$} to 0.3. If the there is no frame with confidence greater or equal than the set $\bm{c}_{max}$, the max confidence of frames in the video is used as $\bm{c}_{max}$.
\textcolor{blue}{$\bm{c}_{min}$} is set to 
\textcolor{blue}{$\bm{c}_{max}$  - 0.1}.
The retrieval time for all 10k videos in \textcolor{blue}{ATBS} dataset is around 23 hours.

For the question answering end-to-end training, we use a VideoQA model ALPRO \cite{li2022align_alpro} for answer prediction and adopted the same setting as the offline 
method for comparison except that our sample range for frames is localized using our algorithm in an online setting while the offline method can access the whole video as the sample range. Both of the methods takes in 4 frames randomly sampled from the sample range. 
The initial learning rate is set to 5e-5 and linearly decayed in the following epochs. The training batch size is 48. The AdamW is used as the optimizer
with a weight decay of 1e-3. A single NVIDIA A100 GPU is used to performed all the experiments. Both of the methods takes about 3 GPU hours to train 20 epochs.

\subsection{Comparison with the Existing Dataset}
As Table \ref{tab:2}. shown, the baseline model outperform the accuracy on MSVD-QA \cite{xu2017video_att_MSVD-QA_MSRVTT-QA_end-to-end_attention_model} and MSRVTT-QA \cite{xu2017video_att_MSVD-QA_MSRVTT-QA_end-to-end_attention_model} much higher than our dataset (ATBS). It demonstrates that ATBS is more challenging than MSVQ-QA and MSRVTT-QA, which consistent to our expectation. Due to MSRVTT-QA as target event in our dataset generation,  it also can prove the effectiveness of our background + target approach.
%

    % "overall_acc": 45.94,
    % "what_acc": 37.05,
    % "who_acc": 58.61,
    % "how_acc": 81.62,
    % "where_acc": 46.43,
    % "when_acc": 72.41
    
    % "overall_acc": 42.12,
    % "what_acc": 36.05,
    % "who_acc": 52.24,
    % "how_acc": 85.67,
    % "where_acc": 42.8,
    % "when_acc": 78.88
    
    %[19.16, 33.58, 77.27, 25.00 ,54.55, 24.80]
\begin{table}[ht]
\setlength{\tabcolsep}{1mm}
  \centering
    \begin{tabular}{@{}lcccccc}
%   \begin{tabular}{@{}l p{0.6cm} p{0.6cm} p{0.6cm} p{0.65cm} p{0.6cm} p{0.8cm}}
    \toprule
    Dataset & what & who & how & where & when & overall \\
    \midrule
    MSVD-QA & 37.05 & 58.61 & 81.62 & 46.43 & 72.41 & 45.94    \\
    MSRVTT-QA & 36.05 & 52.24 & 85.67 & 42.80 & 78.88 & 42.12    \\
    \midrule
    \textbf{ATBS} & 19.16 & 33.58 & 77.27 & 25.00 & 54.55 & 24.80 \\
    \bottomrule
    \end{tabular}
    \caption{Comparison with existing VideoQA datasets}
    \label{tab:2}
\end{table}
%



\subsection{Comparison with the Baseline Model}
Figure \ref{fig:3}. shows the results of our methods comparing with the baseline model. Though our method only watch part of the videos, our method still boost the overall performance. These results also demonstrate the effectiveness of our confidence-based target event localization. 
Our method achieved superior results on "What", "Who", and "How" type questions, in which it significantly outperforms the baseline model by  8.1\% on "Who" type questions. This performance indicates our method can locate the target event relevant to human more precisely and give more accurate predictions. 



%%%%%%% Comparison with baseline 

\begin{figure}[htpb]
%\hspace*{1.1cm}
\centering
\includegraphics[width=1\linewidth]{images/results.pdf}
  \caption{Comparison results between the proposed method and baseline model.}
  \label{fig:3}
\end{figure}


% %
% \begin{table}[ht]
%   \centering
%     \begin{tabular}{@{}l | p{0.6cm}  p{0.6cm}  p{0.6cm}  p{0.6cm}  p{0.8cm} | p{0.8cm}}
%     \toprule
%     Methods & what & who & how & where & when & overall \\
%     \midrule
%     Offline & 19.16 &  33.58 & 77.27 & 25.00 & 54.55 & 24.80    \\
%     \midrule
%     \textbf{Online(Ours)} & 19.20 & 41.68 & 79.55 & 25.00 & 54.55 & 27.10 \\
%     \bottomrule
%     \end{tabular}
%     \caption{Comparisons with the offline approach on \textcolor{blue}{ATBS} in top-1 accuracy (\%)}
%     \label{tab:1}
% \end{table}
% %

==> sections/Introduction.tex <==
\section{Introduction}
%outline:
%第一段：1. 随着xx技术的发展，videoQA最近很流行，具体可以利用在xx应用上 2. 有很多这方面的工作，比如说[...]这些人在做cross-modality，[...]这些人在做pre-trained model 3.但是我们观察到video越长预训练效果越差(ALPRO的数据)，这是long-term memory不够，训练样本太少，无效信息占比太高的原因 
%Recent advances in deep neural networks for computer vision and natural language processing facility the vision-language cooperated tasks such as visual question answering (VQA)  \cite{antol2015vqa,shih2016look_vqa}, visual dialog  \cite{das2017visual_dialog,niu2019recursive_dialog}, and video question answering (VideoQA)  \cite{zhao2017video_videoqa,zhu2017uncovering_videoqa,zeng2017leveraging_videoqa}. As a challenging task, VideoQA requires not only the visual and language feature learning but also the cross-modal feature interaction. Many methods have been developed for VideoQA recently, including 1) RNN/Memory-based models, such as co-memory network  \cite{gao2018motion_memory}, heterogeneous memory network  \cite{fan2019heterogeneous_memory}, and augmented memory network  \cite{cai2021feature_memory}; 2) Graph-based models, such as location-aware graph  \cite{huang2020location_graph} and heterogeneous graph  \cite{jiang2020reasoning_graph}; 3) Conditional Relation Network (CRN), such as Hierarchical Condition Relation Networks (HCRN)  \cite{le2020hierarchical_hcrn}, and 4) Attention-based models, such as co-attention-based method  \cite{li2019learnable_coattention,gao2019structured_coattention,zha2019spatiotemporal_coattention} and self-attention-based method  \cite{jin2019multi_selfattention,li2019beyond_selfattention}.

Video Question Answering (VideoQA) helps to quickly acquire necessary information from videos, which is beneficial to various real-life applications, \eg, intelligent conversation \cite{wang2021pairwise_application}, multimedia recommendation \cite{chen2017attentive_multimedia_recommendation, theodoridis2013music_icassp}, and web video summarization \cite{wang2012event_video_summarization,gharbi2017key_icassp}. In open-ended VideoQA tasks, a video and a related question are provided and the model needs to provide the right answer. 
%As the transformer \cite{vaswani2017attention_transformer} succeeds in both computer vision \cite{VIT,liu2021swin_transformer} and natural language processing \cite{devlin-etal-2019-bert}, 
Recent methods \cite{li2019learnable_coattention,gao2019structured_coattention,zha2019spatiotemporal_coattention,jin2019multi_selfattention,li2019beyond_selfattention} often use the attention mechanism to model the interaction between the video and the questions, and have achieved significant progress.



%Promising results though they achieved, most existing methods are faced with problems in real-world applications. 
Almost all the existing models focus on answering questions given short offline videos with a fixed length \cite{}. \rjf{references} But in real-world scenarios, the materials to be analysed can be a video stream from a CCTV or live cast, which means the video can be extremely long and the length is unpredictable, and the video is progressively provided. Online video limits the performance of existing works in 3 aspects: 1) oversized spatial-temporal information that dilutes the density of key features, 2) disturbance events that may confuse the feature encoders, and 3) lack of state updating mechanism that can decide if the information collected is enough for question answering.

To perform video analysis under online cases in real-world applications, we model this new set of video question answering problems as \textbf{O}nline learning in \textbf{V}ideo \textbf{Q}uestion \textbf{A}nswering (OVQA), which is illustrated in Fig \ref{fig:1}. This type of problem refers to a VideoQA problem given a video with unpredictable length and a relevant question. The solver should watch the video from the beginning, terminate when enough information is collected, and answer the question with a human-readable sentence. 
\textcolor{red}{\{Sentences? Figure 1 needs update for consistency with this claim.\}}

\begin{figure*}[htpb]
%\hspace*{1.1cm} 
\centering
\includegraphics[width=0.85\textwidth]{images/Online Video QA Illustration.pdf}
  \caption{
  Illustration of Online Video Question Answering tasks. The length of the video stream is unpredictable so that the solver reads the video stream from the beginning. For each frame input the solver calculates the confidence rate for each candidate answer and decides if the evidence is solid enough to terminate reading.}
  \label{fig:1}
\end{figure*}



%As the success in computer vision and natural language processing, cross-model tasks involving vision and language have emerged as a prospective research topic, such as visual question answering(VQA) \cite{antol2015vqa,shih2016look_vqa}, visual dialog \cite{das2017visual_dialog,niu2019recursive_dialog}, and video question answering(VideoQA) \cite{zhao2017video_videoqa,zhu2017uncovering_videoqa,zeng2017leveraging_videoqa}. 

% Comparing with VQA and visual dialog tasks where language information just about a static image, VideoQA is more challenging due to build the relation in linguistic features, appearance features and motion features, where the video tend to have substantial redundant information especial in temporal level. 

%Related video question answering focus on offline videos. More often, online video stream like surveillance cameras are applied in most situations (ports). In this situation, it is not just implement other VideoQA method in live stream, because there are 1) long temporal information, burden computation 2) disturbance events, effect the accuracy of VideoQA models. Specifically, the Online VideoQA models need to be updated in each small video clip as opposed to batch learning model by watching the entire videos.

%To build the multi-modality connections between visual and text information, most video question answering methods use 1) RNN/Memory-based models, such as co-memory network \cite{gao2018motion_memory}, heterogeneous memory network \cite{fan2019heterogeneous_memory}, and augmented memory network \cite{cai2021feature_memory}. 2) Graph-based models, such as location-aware graph \cite{huang2020location_graph} and heterogeneous graph \cite{jiang2020reasoning_graph}. 3) Conditional Relation Network (CRN), such as Hierarchical Condition Relation Networks (HCRN) \cite{le2020hierarchical_hcrn}. 4) Attention-based models, such as co-attention-based method \cite{li2019learnable_coattention,gao2019structured_coattention,zha2019spatiotemporal_coattention} and self-attention-based method \cite{jin2019multi_selfattention,li2019beyond_selfattention}. While these methods achieve SOTA results in single event without disturbing event happening, there is still a large gap between simple situation and real life with substantial redundant information. 

%Inspired by online video stream and surveillance videos, we introduce a novel \textbf{O}nline learning task in \textbf{V}ideo \textbf{Q}uestion \textbf{A}nswering (OVQA).  

%Confidence-guided temporal shift module
%directional
In this paper, we tackle this problem with an online updating visual-text encoder and a \emph{confidence-guided targeting event localization (CTEL)}. %\textcolor{red}{\{ Consistency? CTEL and CTEM \}}
The motivation of our method is that we use matching values between the given question and receiving video frames to represent the confidence to answer the question. For given video stream, the video-text retrieval for multi-choice questions \cite { ge2022bridging_video_text_retrieval} is performed to calculate the confidence of the question answering in each frame. Simultaneously, the visual encoder is updated by the present frame and the text encoder holds the linguistic information constantly. Once the confidence of the current frame reaches the condition of termination, the visual encoder stops updating and the answer encoder generates reliable answers. Since our method is the first to apply in OVQA task, we modify existing SOTA VideoQA methods \cite{ li2022align_alpro} by allowing for full video encoding. Compared with this baseline, we boost the performance on our dataset. 

We also provide a new dataset for OVQA task. We use Background + Target approach to generate our new dataset \emph{Answer Target in Background Stream (ATBS)} to simulate complex multi-event as wild video streams. Concretely, we choose DiDeMo \cite{anne2017localizing_dataset_ddm} as our background dataset which has 10,464 videos and 
% 26,892 video clips
around 48 seconds average video duration and the video clips from MSRVTT \cite{xu2016msr_dataset} with 10k video clips taken out from 7,180 real world videos 
%collected by real world search engine
with around 14 seconds average duration.
Considering the complexity of temporal levels in real-life situation, we insert the target video clips into the background video streams randomly and assign question answer pairs randomly selected from MSRVTT-QA's \cite{xu2017video_att_MSVD-QA_MSRVTT-QA_end-to-end_attention_model} 243k QA pairs as the annotations. As a result, our dataset contains 10k videos in total with 10k selected QA pairs. We also design experiments to show that our datasets is more challenging than other VideoQA datasets\cite{xu2017video_att_MSVD-QA_MSRVTT-QA_end-to-end_attention_model, xu2016msr_dataset, chen2011collecting_msvd}. 

Our contributions can be summarized as follows: 1) We introduce a novel video question answering task, the Online Video Question Answering (OVQA); 2) we propose a new dataset Answer Target in Background Stream (ATBS) for OVQA; 3) we design a new method with a online updating visual-text encoder and a confidence-guided target event localization to answer the given question in video stream; and 4) the experimental results show that ATBS is challenging for existing method and our proposed method significantly outperforms pipeline.
%第二段：1. 由于在xxx球赛转播等应用里长视频分析的需求，并且我们认为当前的问题和模型无法很好的满足这种需求，我们提出了online video question answering这一个问题 2.问题的定义，提出一个问题，机器在充分长一段video中，通过从前往后看，去理解视频，判断是否收集到足够的信息，停止运行，并回答问题 3. 解答这个问题要求AI在输入接下来一帧或一个segment的时候输出问题的各个答案的置信度，当置信度足够高的时候停止执行 4. 这个问题的评价标准除了accuracy以外，还可以衡量停下来的地方是否正当 5. 和最接近的video retrival相比我们的问题有两大不同，一个是我们的视频长度未知，不能通过branch and bound这样的方法分割原视频，一个是我们要求回答问题
%第三段：1. 为了解决这个新问题，我们设计了一种方法 2. 这个方法用了xx技术建立了一个online update的步骤 3. 介绍你的方法 不要提任何backbone的事情
%第四段：1. 为了测试我们的方法，我们建立了一个新的数据库 2. 建数据库的操作，即随机插帧 3. benchmark建设，之前有的方法为了进行对比，会读入所有video信息再进行问题回答，在和这些方法对比的时候我们只比较accuracy 3. 统计信息，数据库多少视频，多少文本，占磁盘多大，插帧位置分布，插帧长度分布etc 4. 数据会在文章接收后面向公众发布
%第五段：总结我们的contribution 1. 我们定义了online videoQA这个问题 2. 我们为设计了一个baseline方法 3. 我们为了测试效果搭建了一个dataset并提供了benchmark

%介绍online videoqa 与offline videoqa的区别
%1）可以实时地根据现有的帧给出答案，尤其是对于长视频(real-time activity understanding -> complex long-term activity understanding )的情况下，不需要看完整个视频就可以给出答案。应用场景:video stream, Surveillance camera video。2）实时地update模型，online learning: 优化loss -> 优化regret。因此在这篇paper，我们生成了一个包含1W个video的online videoqa dataset， 并且提出了一个方案，取得了SOTA的结果。3) 多条信息造成的干扰，所以需要检索

%related work: offline videoqa; online learning, onlin video understanding: ECO

%our dataset: 
%1) dataset overview: 10000 videos with 10000 question-answer pairs, average length 62s
%2) dataset generation: background video(DiDeMo:10,464 videos,48 second) + target video(MSRVTT: 10,000 videos, 15 seconds), mannual collection -> random insertion
%3) dataset analysis: vs. MSVD-QA, MSRVTT-QA.... longer length

%our method: 
% motivation: complex long-term activity? temporal info? online stream; confidence；not online learning, online update
% overview 1) initial frame localization: question-guided video-text retrieval -> similarity. confidence to answer 2) event localization: Fibonacci series 3) video-text encoding: ALPRO
% experiment/analysis: VS. modified ALPRO, result

%contribution:1) Online videoQA task 2) OVideoQA datasets 3）methods

==> sections/Methods.tex <==
%\textit{[cite]}
%name of the dataset to be defined \textbf{OVQA}
%\textcolor{blue}{}

\section{METHODOLOGY}
\subsection{Overview of Proposed Method}
In this section, we build an online video question answering method via confidence-based target event localization to online update visual-text encoders. It consists of three main modules: 1) Confidence-based Online Visual-Text Encoder. From the outset of the video stream, the confidence to answer related question is updated by the video-text retrieval for multi-choice questions \cite{ge2022bridging_video_text_retrieval} per frame. 
In the video-text retrieval model, the frame encoded in the vision transformer \cite{VIT} is updated by the present frame and the text encoder \cite{sanh2019distilbert} holds the given question throughout.  2) Confidence-based Target Event Localization. Once the confidence of the present frame reach the max expectational confidence \textcolor{red}{need index}, we localize the target event \textcolor{red}{need index} where the confidences of frames meet the minimum expectational confidence \textcolor{red}{need index}. To reduce time complexity, we also bidirectionally traverse the present spatial-temporal space in the Fibonacci sequence. 3) Target-Event-Question Answering. Due to dense video sampling leading to loss of temporal information, we sample target event \textcolor{red}{need index} in the Fibonacci order instead of sampled randomly. Subsequently, the TimeSformer \cite{bertasius2021space_timesformer} and Bert base model \cite{devlin-etal-2019-bert} encodes the sample frames from the target event and the question separately. Furthermore, a reliable answer is generated by the answer decoder \cite{fan2019heterogeneous_HME_mem_att_memory_model_benchmark, le2022hierarchical_HCRN_relation_model_benchmark}.  

%Unlike existing VideoQA models \cite{li2022align_alpro} encoding the whole video, our method can generate reliable answer via watching part of videos. As irrelevant events occurs in video stream irregularly, we use bi-directional confidence-based temporal extension module to localize target event. Then, with the target event random sampled, the visual-text encoder is updated with both target event frames and given questions. 

%The main issue that OVQA raises is that a huge amount of unknown-length and position-irrelevant event information in video stream results in answering the question with less confidence.
%To answer the question based on the target event, we think there should be three steps. 1) The model should skim through the online stream and decide whether the current event is the target event. 2) If the model has enough confidence, the start of the target event should be localized. 3) After the target event is found, one answer module needs to learn to answer the question from the founded event. Based on these, we designed an algorithm for localizing the target event and select a state-of-the-art VideoQA model ALPRO \textit{[cite]} as the answer module. The answer module is online updated in the whole training process.

\subsection{Confidence-based Online Visual-Text Encoder}
Unlike existing VideoQA models \cite{li2022align_alpro, le2022hierarchical_HCRN_relation_model_benchmark,fan2019heterogeneous_HME_mem_att_memory_model_benchmark,xu2017video_att_MSVD-QA_MSRVTT-QA_end-to-end_attention_model} encoding the whole video, online video stream tasks like sports live broadcasts require to answer the given question with low latency in terms of given video frames. In addition, the comprehension of spatial-temporal information for the model is interfered by the events that are irrelevant to the question especially in the verbose videos. Thus, we build confidence-based online visual-text encoder to filter the unrelated events and update our method frame by frame.

To represent the confidence of answering the question, the similarity of the present frame and corresponding question is computed by video-text retrieval for multi-choice questions \cite{ge2022bridging_video_text_retrieval}. In this model, the visual transformer \cite{VIT} takes the present video and outputs visual features. The text transformer \cite{sanh2019distilbert},  a multi-layer bidirectional transformer encoder, encodes linguistic info and outputs text features. Then, the confidence is calculated by the dot product of visual features and text features. As the criteria of the filtering disturbance events, the confidence in the present frame is also the baseline to update the visual-text encoder. \emph{iff} \textcolor{blue}{the confidence of the present frame is less than the expectational confidence, the confidence of the last frame is updated by the present confidence and moved to the next frame otherwise localized range of target event} \textcolor{red}{need index}. Furthermore, the text encoder holds the corresponding question throughout.   

\subsection{Confidence-based Target Event Localization}
Due to the confidence per frame derived from the visual-text retrieval \cite{ge2022bridging_video_text_retrieval}, we design the confidence-based target event localization in the Fibonacci sequence. To more accurately describe the upper and lower limits of the range of target events 
\textcolor{blue}{$\bm{r}_{high}$ and $\bm{r}_{low}$} \textcolor{red}{need index}, 
we set two hyperparameter max expectational confidence 
\textcolor{blue}{$\bm{c}_{max}$} \textcolor{red}{need index} 
and min expectational confidence 
\textcolor{blue}{$\bm{c}_{min}$} \textcolor{red}{need index}. 
Once the confidence of present frame 
\textcolor{blue}{$\bm{c}_{f}$} 
culminates in max expectational confidence 
\textcolor{blue}{$\bm{c}_{max}$} \textcolor{red}{need index}
, we bidirectional traverse with present spatial-temporal space in the Fibonacci sequence and static frames respectively. Since the confidence decrease progressively from max expectational confidence \textcolor{blue}{$\bm{c}_{max}$} \textcolor{red}{need index} 
during the traversal progress, the termination condition is that the confidence of the frame is lower than min expectational confidence \textcolor{blue}{$\bm{c}_{min}$} \textcolor{red}{need index}
. Besides, the video frames traversed are our target event \textcolor{blue}{$\bm{T}$} \textcolor{red}{need index}, which composed of \textcolor{blue}{$\bm{T}_{pre}$} 
and
\textcolor{blue}{$\bm{T}_{aft}$}.
\textcolor{blue}{$\bm{T}_{pre}$}
is the frames traversed before the $f$, including $f$ itself and
\textcolor{blue}{$\bm{T}_{aft}$}
is the frames traversed after the $f$.

%The algorithm for target event localization is shown the \textbf{\textit{pseudocode}.}
%We treat the video in the dataset as an online stream and skim through it using frame skipping technique. More specifically, we skim through the stream 4 frame per seconds. When current frame $f$ is examined, a confidential score $s$ is produced for $f$ to decide if the frame is relevant enough with the question $Q$. Here we use a video-text retrieval model MCQ \textit{[cite]}, which partially pre-trained on multi-choice questions, to match obtain $s$ between current frame $f$ and the question $Q$. we also set a hyper-parameter $c_{forward}$ as the confidence threshold. If $s$ greater than $c_{forward}$, we think the model is confident enough in finding the target event end frame and ready to answer the question. If $s$ always smaller than $c_{forward}$ during the whole video, we treat the frame $f_{max}$ with the max $s$ as the end frame. 

%Then after the end frame $f_{end}$ is located, the forward skimming is stopped and a Fibonacci number based back skim is used to decide the start of the target event. We obtained some confidential scores $b_{p}$ from matching the previous $p$ skimmed frame $f_{p}$ start from the end frame $f_{end} $with the Question $Q$. $p$ is obtained from the fibonacci sequence. For example, we can obtained the previous 3, 5, 7 frame and matched them with Question $Q$ to get $b_{3}$, $b_{5}$, $b_{7}$. We also set another a hyper-parameter $c_{backward}$ as the backward confidence threshold, which is smaller than $c_{forward}$. For current $p$, if $b_{p}$ is smaller than $c_{backward}$, the backward skimming is stopped, $f_{p}$ is considered as the target event start frame $f_{start}$. Otherwise we use the next Fibonacci number continue the same process. We also set an $p_{upper}$ as the backward upper bound to prevent locating frame far before the $f_{end}$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}
  % Template
  \SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
  \SetKwFunction{Union}{Union}\SetKwFunction{FindCompress}{FindCompress}
  \SetKwFunction{Encode}{Encode}
  \SetKwFunction{KeyframeExtraction}{KeyframeExtraction}
  \SetKwFunction{SentencesConstruction}{SentencesConstruction}
  %\emph{}\;
  % Template
  
  % Function used and to be clarified
  \SetKwFunction{VideoTextRetrieval}{VideoTextRetrieval}
  \SetKwFunction{VideoQuestionAnswering}{VideoQuestionAnswering}
  \SetKwFunction{FibonacciNumber}{FibonacciNumber}

  
  %Keyword of Input & Output
  \SetKwInOut{Input}{Inputs}\SetKwInOut{Output}{Output}

  \Input{Online Stream $\bm{O}$ \\
         Question $\bm{q}$ \\
         %Answer Space $A$ 
         }
  \Output{Answer to the question $\bm{\alpha}$}
  \BlankLine
  initialize hyper-parameter $\bm{c}_{max}, \bm{c}_{min}, \bm{r}_{high}, \bm{r}_{low}$\;
  
  \For{ current frame $\bm{f}$ in online stream $\bm{O}$}{

    $\bm{c}_{f}\leftarrow$ \VideoTextRetrieval{$\bm{q}, \bm{f}$}\;
    \eIf{$\bm{c}_{f} \ge \bm{c}_{max}$}{
        $\bm{T}_{pre}\leftarrow$\emph{Dynamically back traverse the frames before $\bm{f}$ based on fibonacci numbers till $\bm{c} < \bm{c}_{min}$}\;
        $\bm{T}_{aft}\leftarrow$ \emph{Statically traverse the frames after $\bm{f}$ with a fixed fibonacci number}\;
        $\bm{T}\leftarrow$ \Union{$\bm{T}_{pre}$ , $\bm{T}_{aft}$}\;
        \textbf{break}\;
    }{
        \textbf{continue}\;
    }
  }
  $\bm{F}\leftarrow$\emph{Randomly sample $\bm{n}$ frames from $\bm{T}$}\;
  $\bm{\alpha}\leftarrow$\VideoQuestionAnswering{q, F}
  
  \caption{Confidence-based Target Event Localization}\label{algo_disjdecomp}
\end{algorithm}
\textcolor{red}{further explanation may needed to describe the code}



\subsection{Target-Event-Question Answering }

When the target event 
\textcolor{blue}{$\bm{T}$} \textcolor{red}{need index} 
is localized, we design frames sampling in the Fibonacci sequence. Comparing selection with internal, random frames sampling may cause too dense frames per unit of time. The worst situation for an arbitrary sample is that most of the selected frames take in an instant, which may be no obvious move within these images. Since the distribution of confidence increases monotonously over time, the integral of the confidence per unit of time decreases from the current time point to the past. Hence, we use frames sampling in the Fibonacci sequence to keep the time cost per unit confidence, instead of static internal. 

The selected frames from the target event and given questions are encoded in TimSformer \cite{bertasius2021space_timesformer} and Bert base model \cite{devlin-etal-2019-bert} respectively. Subsequently, a 6-layer transformer \cite{vaswani2017attention_transformer} is designed to model the attentional information between visual features and linguistic features. Finally, the visual-text features are fused and the answer decoder \cite{fan2019heterogeneous_HME_mem_att_memory_model_benchmark, le2022hierarchical_HCRN_relation_model_benchmark} is adopted to derive the correct answer.

%we pass the question $Q$ and frames between $f_start$ and $f_end$ to an end-to-end state-of-the-art VideoQA model ALPRO to output final predicted answer from answer space. Besides ALPRO's performance, its end-to-end architecture is able to take in variable number of frames and online update model without preserve the frames information.


==> sections/dataset.tex <==
\section{DATASET}
%\textcolor{blue}{ATBS}
%%%%%% Specific Results
\begin{table*}[ht]
  \centering
    \begin{tabular}{@{}lc c c c c c}
    \toprule
                   Dataset & Task    & Video composition   & Duration range & Average duration & \# Videos & \# QA pairs \\
    \midrule
     MSRVTT-QA \cite{xu2017video_att_MSVD-QA_MSRVTT-QA_end-to-end_attention_model} 
                           & VideoQA & Target only         & (9.32s, 30.00s)   & 14s   & 10,000   & 243,680     \\
     MSVD-QA \cite{xu2017video_att_MSVD-QA_MSRVTT-QA_end-to-end_attention_model} 
                           & VideoQA & Target only         & unknown   & 10s   & 1,970   & 50,505  \\
     TGIF-QA \cite{jang2017tgif_dataset} 
                           & VideoQA & Target only         & unknown   & 3s   & 56,720          & 103,919  \\
     Video-QA \cite{zeng2017leveraging_dataset} 
                           & VideoQA & Target only         & unknown   & 45s   & 18,100          & 174,775  \\                       
    \textcolor{blue}{ATBS} & OVQA    & Background + Target & (22.04s, 447.04s) & 63s & 10,000           & 243,680 \\
    \bottomrule
    \end{tabular}
  \caption{ Comparison with Existing VideoQA datasets }
  \label{tab:1}
\end{table*}

We describe our dataset Answer Target in Background Stream (ATBS) in this section as a dataset targeting OVQA tasks. The dataset contains 10k videos in total with 10k question answering pairs. The videos are generated from two publicity available datasets, MSRVTT \cite{xu2016msr_dataset} and DiDeMo \cite{anne2017localizing_dataset_ddm}. The question answering annotations are randomly selected the from MSRVTT-QA's annotations. The proposed datasets is compared with 

%\cite{xu2017video_att_MSVD-QA_MSRVTT-QA_end-to-end_attention_model} automatically %generated from MSRVTT's captions\cite{xu2016msr_dataset.  

\subsection{Data Collection}
%[Design Principles]
Real world video streams generally contains complex temporal information and multiple events. For OVQA in real world video streams, the necessary information needed for correctly answer the question is agnostic and can appear at any random positions in the given video stream with arbitrary duration. To simulate the real-world scene in our dataset \textcolor{blue}{ATBS}, we design a \textbf{Background + Target} approach, where \textbf{Background} is a relative long background video treat as an online video stream and \textbf{Target} is a target video clip with the necessary information needed for answering the given question. For each of the result video in \textcolor{blue}{ATBS}, one \textbf{Background} and one \textbf{Target} are randomly selected from the base datasets and uniquely paired to secure that their lengths are random. Then the \textbf{Target} is inserted into the \textbf{Background} at a random position composing the result video, which secure the random appearance of the needed information in the video stream.

\textbf{Background + Target:}
To simulate the situation more relevant to the real world, where multiple events will appear in a video stream, we choose to use the Distinct Describable Moments (DiDeMo) \cite{anne2017localizing_dataset_ddm} dataset as the source of our background video. Because it has multiple distinct events in each of the dataset video. 
%\textcolor{blue}{its average video length is 48s which is longer than the target clips'  14s average length and} 
For the target video clip, the video clips from MSRVTT \cite{xu2016msr_dataset} are used where each clip is a distinct event. Every video clip from MSRVTT \cite{xu2016msr_dataset} is randomly and uniquely paired with a background video in DiDeMo \cite{anne2017localizing_dataset_ddm} for later result video composition.

\textbf{Target Random Insertion: }
For each paired target video clip and background video, both the target video clip frames and background video frames are resized to $224\times224$. Then the target video clip is directly inserted behind a randomly selected frame in the background video to generate the result video in our dataset. This simulate the random appearance of the target event in the video stream and also keeps a uniform distribution in result videos' target clip locations. 

\textbf{Dataset Generation: }
%In the ideal case, we want the switch between irrelevant parts and the target event to be as smooth as possible. For instance, a sports live streaming in a national stadium are putting camera on jumping events, a athlete wearing black suit jumps first then a athlete wearing red
%suit jumps after. There is a smooth transition between the two events and the live does not have significant change in context. However, manually collecting such videos and annotating them is time consuming and expensive. Therefore, we decided to use random insertion to insert target event clip. Moreover, for relative short background videos (<20 seconds), target clip is directly inserted after a random selected frame.
%For other background videos, target clip is inserted after a random frame selected frame a middle range, prevents target clip appearing at the start or end of the result video.
After all result videos generated, one question answering pair for each of the result video's target clip is randomly selected from MSRVTT-QA \cite{xu2016msr_dataset} question answering pairs. The final dataset contains 10k result videos with the corresponding 10k question answering pairs in total.

\subsection{Dataset analysis}

\begin{figure}[htbp]
\begin{minipage}[t]{0.55\linewidth}
    \includegraphics[width=\linewidth]{images/types_pie.pdf}
    \label{f1}
\end{minipage}%
    \hfill
\begin{minipage}[t]{0.45\linewidth}
    \includegraphics[width=\linewidth]{images/split_pie.pdf}
    \label{f2}
\end{minipage} 
\caption{Distribution of the question types (left) and training split strategy (right) in our dataset.}
\label{tab:3}
\end{figure}

Since there is no OVQA dataset, we compare the main difference between our dataset with the target source dataset, MSRVTT-QA, as shown in Table 1. Both datasets have 10k videos and same question answering annotation distribution. There are 5 types of question in \textcolor{blue}{ATBS} question answering pairs, categorized by the starting word of the question, as shown in Table 2.
The number of the answer space labels is \textcolor{blue}{1290}.
For the dataset split, we select \textcolor{blue}{7K} videos for training set, \textcolor{blue}{1K} video for validation and \textcolor{blue}{2k} video for testing. 

Comparing with other videos in other VideoQA datasets, because \textcolor{blue}{ATBS} is a dataset targeting at OVQA, the average video length for \textcolor{blue}{ATBS} are longer than some VideoQA datasets  \cite{xu2017video_att_MSVD-QA_MSRVTT-QA_end-to-end_attention_model, jang2017tgif_dataset, zeng2017leveraging_dataset} and close to some datasets for temporal localization. The question answering annotations of the \textcolor{blue}{ATBS} dataset have the similar categories as common VideoQA datasets \textcolor{red}{citation} \cite{TVQA}, with the 5 catergories mentioned above. 
%There are no specific modification on question answering pairs, for this work is not aim towards VideoQA in specific domains.

